Quantifying the Variability Collapse of Neural Networks

Recent studies empirically demonstrate the positive relationship between the transferability of neural networks and the within-class variation of the last layer features. The recently discovered Neural Collapse (NC) phenomenon provides a new perspective of understanding such last layer geometry of neural networks. In this paper, we propose a novel metric, named Variability Collapse Index (VCI), to quantify the variability collapse phenomenon in the NC paradigm. The VCI metric is well-motivated and intrinsically related to the linear probing loss on the last layer features. Moreover, it enjoys desired theoretical and empirical properties, including invariance under invertible linear transformations and numerical stability, that distinguishes it from previous metrics. Our experiments verify that VCI is indicative of the variability collapse and the transferability of pretrained neural networks.

==> images/trans_prev.tex <==
\begin{figure*}[t]
     \centering
     \begin{subfigure}
         \centering
         \includegraphics[width=0.32\textwidth]{images/rn50_temptrans_fuz.pdf}
     \end{subfigure}
     \hfill
     \begin{subfigure}
         \centering
         \includegraphics[width=0.32\textwidth]{images/rn50_temptrans_sq.pdf}
     \end{subfigure}
     \hfill
     \begin{subfigure}
         \centering
         \includegraphics[width=0.32\textwidth]{images/rn50_temptrans_cs.pdf}
     \end{subfigure}
     \\
          \centering
     \begin{subfigure}
         \centering
         \includegraphics[width=0.32\textwidth]{images/rn50_l4trans_fuz.pdf}
     \end{subfigure}
     \hfill
     \begin{subfigure}
         \centering
         \includegraphics[width=0.32\textwidth]{images/rn50_l4trans_sq.pdf}
     \end{subfigure}
     \hfill
     \begin{subfigure}
         \centering
         \includegraphics[width=0.32\textwidth]{images/rn50_l4trans_cs.pdf}
     \end{subfigure}
        \caption{A negative relation between previous variability metrics and transferability can be observed when changing the temperature of softmax in pretraining. However, a nearly opposite trend emerges when we adjust the weight of Cosine Similarity regularization term. Architecture: ResNet50. Dataset: ImageNet-1K. The mean log odd is calculated over 10 downstream datasets.}
        \label{fig: trans_prev}
\end{figure*}


==> images/vc_col.tex <==
\begin{figure*}[t]
     \centering
     \begin{subfigure}
         \centering
         \includegraphics[width=0.32\textwidth]{images/rn50_vc.pdf}
     \end{subfigure}
     \hfill
     \begin{subfigure}
         \centering
         \includegraphics[width=0.32\textwidth]{images/rn18_vc.pdf}
     \end{subfigure}
     \hfill
     \begin{subfigure}
         \centering
         \includegraphics[width=0.32\textwidth]{images/deit_vc.pdf}
     \end{subfigure}
        \caption{Our proposed metric VC consistently decrease as training proceeds across various network architectures and training settings. Left: ResNet50. Middle: ResNet18. Right: DeiT.}
        \label{fig: vc_col}
\end{figure*}


==> images/vc_trans.tex <==
\begin{figure*}[t]
     \centering
     \begin{subfigure}
         \centering
         \includegraphics[width=0.48\textwidth]{images/rn50_temptrans_vc.pdf}
     \end{subfigure}
     \hfill
     \begin{subfigure}
         \centering
         \includegraphics[width=0.48\textwidth]{images/rn50_l4trans_vc.pdf}
     \end{subfigure}
        \caption{Our proposed metric VC has a consistent relation with transferability in our experiments. Left: Different values of temperature of the softmax. Right: Different values of the $\lambda$-coefficient of Similarity Regularization.}
        \label{fig: vc_trans}
\end{figure*}


==> text_old/Appropriate.tex <==
\section{What is an Appropriate Variability Collapse Metric?}

We discuss in this section from several aspects that the previous variability collapse metrics are not perfect, and propose our novel metric to solve the issues.

\subsection{Do Last Layer Features Really Collapse?}

In~\citet{prevalence}, NC1, or Variability Collapse, is stated as `\dots the
within-class variation of the activations becomes negligible \dots', with a mathematical version $\Sigma_W \rightarrow 0$ lacking clarification of in what sense the convergence holds. We point out that even the fuzziness reaches 0, the within-class variation is in general `non-negligible', in the sense that the representation is far from what they depicted in the `balls-and-sticks' graph \cref{fig: nc1balls}.

We show the following fact.
\begin{proposition}\label{lem: fuz no collapse}
Assume $p \geq K$. For any fixed frame $\{\mu_k\}_{k\in[K]}$ that is not all equal, the Squared Distance (\cref{eq: mean var}), or $\Norm{\Sigma_W}_F$ can be arbitrary large under $\Tr(\Sigma_B^\dagger\Sigma_W) = 0$.  
\end{proposition}
\begin{proof}[Proof of Lemma~\ref{VC-inv}]
Denote $V_B = \spn(\{\mu_1 - \mu_G, \cdots, \mu_K - \mu_G\})$.
Note that by $\mu_G = \sum_{k=1}^K \frac{n_k}{n}\mu_k$, we have
\begin{align*}
    \sum_{k=1}^K \frac{n_k}{n}(\mu_k - \mu_G) = 0,
\end{align*}
which leads to $\operatorname{rank}(\Sigma_B) \leq K - 1 < p$. This indicates a non-empty orthogonal complement of $V_B$. Let $U_1$ be an and $U_2$ consist of 
\end{proof}

We say a neural representation achieves \newterm{full collapse} if $\Sigma_W = 0$. The above result shows 0 fuzziness only guarantees \newterm{partial collapse} in $V_B$ and the variance corresponding to $V_B^\perp$ is not constrained. On the contrary, the Squared Distance attains $0$ if and only if $\Norm{\Sigma_W}_F = 0$. As to Cosine Similarity, although its variance in $V_B^\perp$ is constrained, achieving 0 still does not mean full collapse.

\input{images/rn18_col.tex}
\input{images/rn50_col.tex}

We show that, such differences in these collapse metrics can result in different trends exhibited in training neural networks. \cref{fig: rn18_col} shows that for resnet18 trained on cifar10, in common training settings, both Squared Distance and Cosine Similarity do not collapse sometimes. This can be mainly attributed to the increase of $V_B^\perp$ part of variability, as we can see in \cref{fig: rn18_sqout}. 
\begin{figure}[h]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=0.9\columnwidth]{images/rn18_sqout.pdf}}
\caption{The projection of squared distance onto $V_B^\perp$ during the training of ResNet18 on Cifar10. The curves correspond to the ones in \cref{fig: rn18_col}.}
\label{fig: rn18_sqout}
\end{center}
\vskip -0.2in
\end{figure}

For ResNet50 trained on ImageNet-1k, \cref{fig: rn50_col} shows that all three metrics maintain to collapse in the experimented training settings. Nevertheless, the $V_B^\perp$ part can still increase when the network is trained with cross-entropy loss, as we can see in \cref{fig: rn50_sqout}. Due to this part is small in this $p/K \sim 2$ setting, it does not affect the whole trend.

\begin{figure}[h]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=0.9\columnwidth]{images/rn50_sqout.pdf}}
\caption{The projection of squared distance onto $V_B^\perp$ during the training of ResNet50 on ImageNet-1k. The curves correspond to the ones in \cref{fig: rn50_col}.}
\label{fig: rn50_sqout}
\end{center}
\vskip -0.2in
\end{figure}


% Conclusion: even in common training settings, Belkin and cos sim can fail to show the trend of collapse, due to the increase of $V_{B}^\perp$ part of variance. To put it another way, the reason fuzziness maintains to decrease is that ignores the variability in $V_B^\perp$, as a result of which, 0 fuzziness does not mean the neural representation approaches Full Collapse. 

Such results are not surprising, considering the following fact:
\begin{proposition}\label{lem: nc3VB}
If NC3 holds, then for any loss function $L(Z)$ defined on the logits $Z = WH + b1_n^T$, $L = 0$ adds no constraint on variability in $V_B^\perp$.
\end{proposition}
\begin{proof}
    $W^T = M$.
\end{proof}

As a result, variability metrics that can exhibit full collapse might be undesirable, if our goal is to obtain a consistent conclusion on the structural property of pretrained neural representation across different network structures and training datasets, despite that such notions seem more consistent with our intuitions at first glance.

%Furthermore, we show that by add some simple regularization, we can train neural networks that do not collapse in any these metrics, with almost the same performance. This result indicates that variability collapse might have limited explain-ability for the success of modern deep neural networks on classification tasks.

\subsection{Do variability collapse metrics indeed indicate better transferability?}
When faced with a set of similar notions, we should always choose the most useful one. One usage of variability collapse metrics is to indicate the transferability of neural representation, as suggested in \citep{hui2022limitations, kornblith2021better}. 

We use log odd gain to measure how well a neural representation transfer compared to its performance on the dataset for pretraining. 

\input{images/trans_prev.tex}
As shown in the top row \cref{fig: trans_prev}, we verify that a negative relation between variability collapse and tranferability can be observed when we change some of the hyperparameters. However, we can find training settings where the relation turns to be positive. We add Cosine Similarity calculated on each batch as an regularization term during training. In the bottom row of \cref{fig: trans_prev}, we see that the cos-sim regularized neural networks show consistent high values for these metrics while transfer worse.

\subsection{Invariance under invertible linear transformations matters}
We argue that invariance under invertible linear transformations is a necessary Condition for fair compare between two neural representations.

The loss function is invariant under invertible linear transformation.

We propose our novel variability collapse metric, simply denoted by VC, with the form
\begin{equation}\label{VC-exp}
    \operatorname{VC}= 1 - \frac{\Tr[\Sigma_B(\Sigma_T)^\dagger]}{\operatorname{rank}(\Sigma_B)}.
\end{equation}


\begin{lemma}\label{VC-inv}
$\operatorname{VC}$ is invariant under any invertible linear transformation.
\end{lemma}
\begin{proof}[Proof of Theorem~\ref{VC-inv}]
 Let $N$ denote the matrix attained by subtracting each row of $H$ by the corresponding class-mean $\mu_k = \sum_{i\in[n_k]}h_{k, i}$. Let $r$ denote the rank of $\Sigma_T$. By
 \begin{align*}
 \Sigma_T = (N^T|M^T) \begin{pmatrix},
 N \\ M
 \end{pmatrix}
 \end{align*}
 we know that the span of the singular vectors $\{u_k\}_{k=1}^r$ of $\Sigma_T$ contains $\Sigma_{T} = \spn(M^T)$. Thus,
 \begin{equation*}
     UU^T\Sigma_B UU^T = \Sigma_B,
 \end{equation*}
 where $U = (u_1, \cdots, u_r)$. For any invertible linear transformation $A$, $AU$ has the representation $U_AR_A$, where $U_A \in \BR^{p\times r}$ has orthonormal columns and $R_A \in \BR^{r\times r}$ is of full rank. The conclusion follows by
\begin{align*}
&\Tr[A\Sigma_B A^T(A\Sigma_T A^T)^\dagger] \\
= &\Tr[AUU^T\Sigma_B UU^TA^T(AU\Lambda_TU^TA^T)^\dagger] \\
= &\Tr[U_AR_AU^T\Sigma_BUR_A^TU_A^TU_A(R_A\Lambda_TR_A^T)^{-1}U_A^T] \\
=& \Tr[U^T\Sigma_BU\Lambda_T^{-1}] \\
=& \Tr[\Sigma_B(\Sigma_T)^\dagger].
\end{align*}

\end{proof}

\input{images/vc_col.tex}
\input{images/vc_trans.tex}

Our experiments show that VC, to our expectation, consistently decrease during pretraining in common training settings, as shown in . Surprisingly, by 



\subsection{Numerical issues}
We shall point out Another pitfall of fuzziness is its instability in numerical calculation. The choice of tolerance in calculating the pseudo-inverse term in fuzziness can be very tricky. For calculation using 32bit float point, the gap between the minimum eigenvalue and the largest eigenvalue that 'is supposed to be 0' can be as small as around only 2 magnitude of scales. In contrast, the nonzero eigenvalues can be distributed in a range larger than 5 magnitude of scales. This makes it difficult to select an appropriate tolerance value for the pseudo-inverse operation in advance. For example, in our experiments, when we use the default tolerance provided by PyTorch~\citep{paszke2019pytorch}, sometimes 20 percent of the nonzero eigenvalues will be treated as zero. One may partly avoid this issue when $p \geq K$ by instead performing singular value decomposition for $M$, the matrix whose rows are the global-centered class-means $\{\mu_k\}_{k\in[K]}$. The last singular value should always be treated as 0 since the global mean is on the simplex of class-means, while the others might still face the same issue.

Even in the $p < K$ case (which is the case of ViT-based structures on ImageNet), we have encountered cases where the first $p-1$ singular values are in the scale of $1$ to $50$ while the last singular value happens to be around 1e-6. See \cref{exp: degenerate} for a discussion of why such situation can happen. 

Anyway, this issue comes from the fact that, there is no \emph{a prior principle} of when to abandon small singular values when calculating the fuzziness, unless we have investigated into the intrinsic structure theoretically. In contrast, our VC metric is free of such issue due to the relation between $V_B$ and $V_T$. 
 
\subsection{Summary}

We summary the key properties of the different variability in \cref{tab: metric}. The columns shows
\begin{itemize}
    \item Invariant: invariance under invertible linear transformation.
    \item Collapse: whether this metric exhibit the trend of collapse in common training settings.
    \item Stability: numerical stability.
    \item Full Collapse: Whether 0 metric value means Full collapse in the feature space.
    \item Trans: whether the metric is indicative of the transfer performance.
\end{itemize}
\begin{table*}[t]
\caption{Properties of the discussed variability collapse metric}
\label{tab: metric}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lccccc}
\toprule
Metric & Invariant & Collapse? & Stability &Full Collapse & Trans \\
\midrule
Fuzziness      & in $V_B$&  $\surd$& $\Delta$ & $\Delta$ &$\Delta$ \\
Cos Similarity  & $\times$& $\Delta$&  $\surd$& $\Delta$ &$\Delta$ \\
Squared Distance & $\times$& $\Delta$&  $\surd$& $\surd$  &$\Delta$ \\
VC(Ours) & $\surd$ &  $\surd$& $\surd$ & $\surd$ &$\surd$  \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}

We believe that 

==> text_old/intro_another.tex <==
\section{Introduction}
Understanding neural representation is important.

Neural Collapse receives much attention recently. But no thorough discussion on the variability metric. There are different ones.

We first do a in-depth investigation on what are the desired properties for an ideal variability collapse metric.

We also find that our proposed metric indicates transferability when the previous metrics fail. 
